Compositional Safety Verification with Max-SMT

We present an automated compositional program verification technique for safety properties based on conditional inductive invariants. For a given program part (e.g., a single loop) and a postcondition $\varphi$, we show how to, using a Max-SMT solver, an inductive invariant together with a precondition can be synthesized so that the precondition ensures the validity of the invariant and that the invariant implies $\varphi$. From this, we build a bottom-up program verification framework that propagates preconditions of small program parts as postconditions for preceding program parts. The method recovers from failures to prove the validity of a precondition, using the obtained intermediate results to restrict the search space for further proof attempts. As only small program parts need to be handled at a time, our method is scalable and distributable. The derived conditions can be viewed as implicit contracts between different parts of the program, and thus enable an incremental program analysis.

==> experiments.tex <==
%\begin{landscape}
\section{Experiments}
\label{sec:Experiments}

In the following, we display detailed results for the examples from
the \tool{HOLA} benchmark suite. A \checkmark\ in the ``Result''
column means that we could successfully prove all properties asserted
for the example program (column ``Property'').
 The runtime is measured in seconds, and corresponds to the
\emph{sequential} version of \tool{VeryMax-Seq}. We also report the number of
calls to the \checkSafe{} procedure and the maximal nesting level of such
calls. Finally, the last two columns display the runtime (in seconds) spent in
the SMT solving backend, split between queries that are satisfiable and those
that are unsatisfiable. Note that unsatisfiable queries have the most
significant contribution to the overall runtime. We speculate that an SMT prover
with better support for UNSAT proofs could speed up the overall method
significantly.

%\vspace{0.2cm}

%%\begin{longtable}{|l|c|r|r|r|r|r|r|}
%%  \hline
%%   Example & Result & Runtime & Property & Calls & Depth & \textbf{R} (SAT) & \textbf{R} (UNSAT)\\\hline
%%   \endhead
%%   \multirow{1}{*}{01.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.02} &
%%     \texttt{1 <= \_Z6mymainv\_y} &
%%     1 &
%%     0 &
%%     0.01 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{02.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.13} &
%%     \texttt{\_Z6mymainv\_x <= \_Z6mymainv\_y} &
%%     1 &
%%     0 &
%%     0.01 &
%%     0.00 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_y <= \_Z6mymainv\_x} &
%%     1 &
%%     0 &
%%     0.03 &
%%     0.08 \\
%% \hline
%%   \multirow{1}{*}{03.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{1.39} &
%%     \texttt{1 <= \_Z6mymainv\_i} &
%%     2 &
%%     1 &
%%     0.61 &
%%     0.76 \\
%% \hline
%%   \multirow{1}{*}{04.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.01} &
%%     \texttt{1 <= \_Z6mymainv\_y} &
%%     3 &
%%     2 &
%%     0.01 &
%%     0.00 \\
%% \hline
%%   \multirow{1}{*}{05.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.11} &
%%     \texttt{\_Z6mymaini\_i <= \_Z6mymaini\_j} &
%%     2 &
%%     1 &
%%     0.06 &
%%     0.05 \\
%% \hline
%%   \multirow{2}{*}{06.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.43} &
%%     \texttt{\_Z6mymainv\_x <= \_Z6mymainv\_y} &
%%     1 &
%%     0 &
%%     0.05 &
%%     0.14 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_y <= \_Z6mymainv\_x} &
%%     1 &
%%     0 &
%%     0.06 &
%%     0.13 \\
%% \hline
%%   \multirow{2}{*}{07.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.56} &
%%     \texttt{\_Z6mymainv\_a + \_Z6mymainv\_b <= 3*\_Z6mymainv\_n} &
%%     3 &
%%     2 &
%%     0.21 &
%%     0.32 \\
%%     & & &
%%     \texttt{3*\_Z6mymainv\_n <= \_Z6mymainv\_a + \_Z6mymainv\_b} &
%%     2 &
%%     1 &
%%     0.03 &
%%     0.00 \\
%% \hline
%%   \multirow{1}{*}{08.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.33} &
%%     \texttt{3 <= \_Z6mymainv\_y} &
%%     2 &
%%     1 &
%%     0.01 &
%%     0.31 \\
%% \hline
%%   \multirow{1}{*}{09.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{11.06} &
%%     \texttt{0 <= \_Z6mymainv\_k} &
%%     16 &
%%     3 &
%%     0.69 &
%%     10.14 \\
%% \hline
%%   \multirow{2}{*}{10.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.50} &
%%     \texttt{\_Z6mymainv\_x <= \_Z6mymainv\_y} &
%%     1 &
%%     0 &
%%     0.01 &
%%     0.19 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_y <= \_Z6mymainv\_x} &
%%     1 &
%%     0 &
%%     0.01 &
%%     0.19 \\
%% \hline
%%   \multirow{3}{*}{11.c} &
%%   \multirow{3}{*}{\checkmark} &
%%   \multirow{3}{*}{3.31} &
%%     \texttt{\_Z6mymainv\_j <=200} &
%%     2 &
%%     1 &
%%     0.00 &
%%     1.81 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_j <=200} &
%%     2 &
%%     1 &
%%     0.73 &
%%     0.77 \\
%%     & & &
%%     \texttt{200 <= \_Z6mymainv\_j} &
%%     2 &
%%     1 &
%%     0.01 &
%%     0.00 \\
%% \hline
%%   \multirow{1}{*}{12.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{5.09} &
%%     \texttt{\_Z6mymaini\_y <=4} &
%%     9 &
%%     3 &
%%     1.49 &
%%     3.47 \\
%% \hline
%%   \multirow{2}{*}{13.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{1.95} &
%%     \texttt{\_Z6mymaini\_j <= 2 + 2*\_Z6mymaini\_k} &
%%     6 &
%%     2 &
%%     0.92 &
%%     0.87 \\
%%     & & &
%%     \texttt{2 + 2*\_Z6mymaini\_k <= \_Z6mymaini\_j} &
%%     3 &
%%     1 &
%%     0.06 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{14.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{1.58} &
%%     \texttt{0 <= \_Z6mymainv\_a + \_Z6mymainv\_m} &
%%     2 &
%%     1 &
%%     0.02 &
%%     0.76 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_a <= \_Z6mymainv\_m} &
%%     2 &
%%     1 &
%%     0.03 &
%%     0.77 \\
%% \hline
%%   \multirow{1}{*}{15.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.77} &
%%     \texttt{0 <= \_Z6mymainv\_k} &
%%     2 &
%%     1 &
%%     0.02 &
%%     0.76 \\
%% \hline
%%   \multirow{2}{*}{16.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.01} &
%%     \texttt{\_Z6mymainii\_y <=0} &
%%     2 &
%%     1 &
%%     0.01 &
%%     0.00 \\
%%     & & &
%%     \texttt{0 <= \_Z6mymainii\_y} &
%%     2 &
%%     1 &
%%     0.01 &
%%     0.00 \\
%% \hline
%%   \multirow{1}{*}{17.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.86} &
%%     \texttt{\_Z6mymaini\_n <= \_Z6mymaini\_k} &
%%     3 &
%%     2 &
%%     0.10 &
%%     0.76 \\
%% \hline
%%   \multirow{2}{*}{18.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{4.63} &
%%     \texttt{\_Z6mymainii\_j <=100} &
%%     6 &
%%     2 &
%%     1.97 &
%%     2.28 \\
%%     & & &
%%     \texttt{100 <= \_Z6mymainii\_j} &
%%     3 &
%%     1 &
%%     0.29 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{19.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{3.73} &
%%     \texttt{\_Z6mymainii\_y <= \_Z6mymainii\_n} &
%%     6 &
%%     2 &
%%     0.92 &
%%     2.26 \\
%%     & & &
%%     \texttt{\_Z6mymainii\_n <= \_Z6mymainii\_y} &
%%     3 &
%%     2 &
%%     0.04 &
%%     0.32 \\
%% \hline
%%   \multirow{4}{*}{20.c} &
%%   \multirow{4}{*}{\checkmark} &
%%   \multirow{4}{*}{2.95} &
%%     \texttt{\_Z6mymainiiiiii\_x + \_Z6mymainiiiiii\_y <= \_Z6mymainiiiiii\_k} &
%%     2 &
%%     1 &
%%     0.03 &
%%     0.00 \\
%%     & & &
%%     \texttt{\_Z6mymainiiiiii\_k <= \_Z6mymainiiiiii\_x + \_Z6mymainiiiiii\_y} &
%%     2 &
%%     1 &
%%     0.02 &
%%     0.00 \\
%%     & & &
%%     \texttt{0 <= \_Z6mymainiiiiii\_m} &
%%     4 &
%%     3 &
%%     0.08 &
%%     0.35 \\
%%     & & &
%%     \texttt{1 + \_Z6mymainiiiiii\_m <= \_Z6mymainiiiiii\_n} &
%%     7 &
%%     3 &
%%     0.36 &
%%     1.84 \\
%% \hline
%%   \multirow{1}{*}{21.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.02} &
%%     \texttt{1 + \_Z6mymainv\_n <= \_Z6mymainv\_k} &
%%     2 &
%%     1 &
%%     0.02 &
%%     0.00 \\
%% \hline
%%   \multirow{4}{*}{22.c} &
%%   \multirow{4}{*}{\checkmark} &
%%   \multirow{4}{*}{0.11} &
%%     \texttt{\_Z6mymainv\_x <= \_Z6mymainv\_y} &
%%     1 &
%%     0 &
%%     0.01 &
%%     0.00 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_y <= \_Z6mymainv\_x} &
%%     1 &
%%     0 &
%%     0.05 &
%%     0.02 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_y <= \_Z6mymainv\_z} &
%%     1 &
%%     0 &
%%     0.01 &
%%     0.00 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_z <= \_Z6mymainv\_y} &
%%     1 &
%%     0 &
%%     0.01 &
%%     0.00 \\
%% \hline
%%   \multirow{1}{*}{23.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.32} &
%%     \texttt{0 <= \_Z6mymaini\_sum} &
%%     3 &
%%     2 &
%%     0.01 &
%%     0.30 \\
%% \hline
%%   \multirow{1}{*}{24.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.30} &
%%     \texttt{\_Z6mymainv\_i <= \_Z6mymainv\_k} &
%%     2 &
%%     1 &
%%     0.24 &
%%     0.04 \\
%% \hline
%%   \multirow{1}{*}{25.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.12} &
%%     \texttt{\_Z6mymainv\_j <= \_Z6mymainv\_i} &
%%     1 &
%%     0 &
%%     0.05 &
%%     0.06 \\
%% \hline
%%   \multirow{2}{*}{26.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.58} &
%%     \texttt{\_Z6mymainv\_x <= \_Z6mymainv\_y} &
%%     1 &
%%     0 &
%%     0.07 &
%%     0.18 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_y <= \_Z6mymainv\_x} &
%%     1 &
%%     0 &
%%     0.08 &
%%     0.17 \\
%% \hline
%%   \multirow{1}{*}{27.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.02} &
%%     \texttt{1 <= \_Z6mymainv\_k} &
%%     1 &
%%     0 &
%%     0.02 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{28.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.03} &
%%     \texttt{\_Z6mymainv\_y <=0} &
%%     3 &
%%     2 &
%%     0.01 &
%%     0.00 \\
%%     & & &
%%     \texttt{0 <= \_Z6mymainv\_y} &
%%     3 &
%%     2 &
%%     0.01 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{29.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.15} &
%%     \texttt{\_Z6mymainv\_a + \_Z6mymainv\_c <= \_Z6mymainv\_b + \_Z6mymainv\_d} &
%%     1 &
%%     0 &
%%     0.02 &
%%     0.00 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_b + \_Z6mymainv\_d <= \_Z6mymainv\_a + \_Z6mymainv\_c} &
%%     1 &
%%     0 &
%%     0.05 &
%%     0.07 \\
%% \hline
%%   \multirow{1}{*}{30.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.77} &
%%     \texttt{0 <= \_Z6mymainv\_c} &
%%     2 &
%%     1 &
%%     0.02 &
%%     0.75 \\
%% \hline
%%   \multirow{2}{*}{31.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{2.71} &
%%     \texttt{0 <= \_Z6mymainv\_j} &
%%     2 &
%%     1 &
%%     0.61 &
%%     0.74 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_i <= 4 + \_Z6mymainv\_j + \_Z6mymainv\_n} &
%%     1 &
%%     0 &
%%     0.51 &
%%     0.75 \\
%% \hline
%%   \multirow{2}{*}{32.c} &
%%   \multirow{2}{*}{\text{\sffamily X}} &
%%   \multirow{2}{*}{5.25} &
%%     \texttt{\_Z6mymainv\_i <= \_Z6mymainv\_j} &
%%     5 &
%%     2 &
%%     0.40 &
%%     2.14 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_i <= \_Z6mymainv\_j} &
%%     5 &
%%     2 &
%%     0.41 &
%%     2.16 \\
%% \hline
%%   \multirow{2}{*}{33.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.23} &
%%     \texttt{\_Z6mymaini\_x <= \_Z6mymaini\_y} &
%%     1 &
%%     0 &
%%     0.02 &
%%     0.17 \\
%%     & & &
%%     \texttt{\_Z6mymaini\_y <= \_Z6mymaini\_x} &
%%     1 &
%%     0 &
%%     0.02 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{34.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.09} &
%%     \texttt{\_Z6mymaini\_x <= 2*\_Z6mymaini\_y} &
%%     2 &
%%     1 &
%%     0.05 &
%%     0.00 \\
%%     & & &
%%     \texttt{2*\_Z6mymaini\_y <= \_Z6mymaini\_x} &
%%     2 &
%%     1 &
%%     0.04 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{35.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.01} &
%%     \texttt{\_Z6mymaini\_x <= \_Z6mymaini\_n} &
%%     3 &
%%     2 &
%%     0.01 &
%%     0.00 \\
%%     & & &
%%     \texttt{\_Z6mymaini\_n <= \_Z6mymaini\_x} &
%%     2 &
%%     1 &
%%     0.00 &
%%     0.00 \\
%% \hline
%%   \multirow{3}{*}{36.c} &
%%   \multirow{3}{*}{\checkmark} &
%%   \multirow{3}{*}{9.24} &
%%     \texttt{\_Z6mymaini\_z <= \_Z6mymaini\_w} &
%%     2 &
%%     1 &
%%     0.15 &
%%     0.35 \\
%%     & & &
%%     \texttt{\_Z6mymaini\_a <= \_Z6mymaini\_b} &
%%     4 &
%%     2 &
%%     0.56 &
%%     2.97 \\
%%     & & &
%%     \texttt{\_Z6mymaini\_b <= \_Z6mymaini\_a} &
%%     4 &
%%     2 &
%%     0.73 &
%%     3.60 \\
%% \hline
%%   \multirow{2}{*}{37.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.88} &
%%     \texttt{0 <= \_Z6mymaini\_m} &
%%     3 &
%%     2 &
%%     0.05 &
%%     0.79 \\
%%     & & &
%%     \texttt{1 + \_Z6mymaini\_m <= \_Z6mymaini\_n} &
%%     2 &
%%     1 &
%%     0.03 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{38.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.09} &
%%     \texttt{\_Z6mymaini\_x <= 2*\_Z6mymaini\_y} &
%%     2 &
%%     1 &
%%     0.05 &
%%     0.00 \\
%%     & & &
%%     \texttt{2*\_Z6mymaini\_y <= \_Z6mymaini\_x} &
%%     2 &
%%     1 &
%%     0.05 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{39.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.81} &
%%     \texttt{0 <= \_Z6mymainv\_glob3\_dc} &
%%     1 &
%%     0 &
%%     0.00 &
%%     0.00 \\
%%     & & &
%%     \texttt{\_Z6mymainv\_glob3\_dc <= MAXPATHLEN} &
%%     1 &
%%     0 &
%%     0.06 &
%%     0.75 \\
%% \hline
%%   \multirow{2}{*}{40.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{12.09} &
%%     \texttt{\_Z6mymaini\_a <= \_Z6mymaini\_b} &
%%     11 &
%%     3 &
%%     0.54 &
%%     5.19 \\
%%     & & &
%%     \texttt{\_Z6mymaini\_b <= \_Z6mymaini\_a} &
%%     9 &
%%     3 &
%%     0.96 &
%%     3.92 \\
%% \hline
%%   \multirow{1}{*}{41.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.78} &
%%     \texttt{1 + 2*\_Z6mymainii\_n <= \_Z6mymainii\_z} &
%%     2 &
%%     1 &
%%     0.03 &
%%     0.75 \\
%% \hline
%%   \multirow{2}{*}{42.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{13.16} &
%%     \texttt{\_Z6mymaini\_a = 1 + 2*q\_div\_2\_\_Z6mymaini\_a\_id11} &
%%     11 &
%%     2 &
%%     1.00 &
%%     10.88 \\
%%     & & &
%%     \texttt{1 + \_Z6mymaini\_a = 2*q\_div\_2\_\_Z6mymaini\_a\_id11} &
%%     4 &
%%     1 &
%%     0.28 &
%%     0.00 \\
%% \hline
%%   \multirow{1}{*}{43.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.00} &
%%     \texttt{\_Z6mymainii\_t <= \_Z6mymainii\_y} &
%%     1 &
%%     0 &
%%     0.00 &
%%     0.00 \\
%% \hline
%%   \multirow{2}{*}{44.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{1.69} &
%%     \texttt{\_Z6mymainii\_j <= \_Z6mymainii\_i} &
%%     5 &
%%     2 &
%%     0.07 &
%%     0.76 \\
%%     & & &
%%     \texttt{\_Z6mymainii\_i <= \_Z6mymainii\_j} &
%%     2 &
%%     1 &
%%     0.08 &
%%     0.76 \\
%% \hline
%%   \multirow{2}{*}{45.c} &
%%   \multirow{2}{*}{\checkmark} &
%%   \multirow{2}{*}{0.72} &
%%     \texttt{\_Z6mymaini\_x <= \_Z6mymaini\_y} &
%%     3 &
%%     2 &
%%     0.17 &
%%     0.24 \\
%%     & & &
%%     \texttt{\_Z6mymaini\_y <= \_Z6mymaini\_x} &
%%     1 &
%%     0 &
%%     0.05 &
%%     0.17 \\
%% \hline
%%   \multirow{1}{*}{46.c} &
%%   \multirow{1}{*}{\checkmark} &
%%   \multirow{1}{*}{0.53} &
%%     \texttt{\_Z6mymainv\_x <=1} &
%%     1 &
%%     0 &
%%     0.20 &
%%     0.32 \\
%% \hline
%% \end{longtable}
\begin{longtable}{|l|c|r|r|r|r|r|r|}
 \hline
  Example & Result & Runtime & Property & Calls & Depth & \textbf{R} (SAT) & \textbf{R} (UNSAT)\\\hline
  \endhead
  \multirow{1}{*}{01} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.02} &
    \texttt{1 <= y} &
    1 &
    0 &
    0.02 &
    0.01 \\
\hline
  \multirow{2}{*}{02} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.20} &
    \texttt{x <= y} &
    1 &
    0 &
    0.02 &
    0.00 \\
    & & &
    \texttt{y <= x} &
    1 &
    0 &
    0.09 &
    0.07 \\
\hline
  \multirow{1}{*}{03} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{2.12} &
    \texttt{1 <= i} &
    2 &
    1 &
    0.98 &
    1.12 \\
\hline
  \multirow{1}{*}{04} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.02} &
    \texttt{1 <= y} &
    3 &
    2 &
    0.02 &
    0.00 \\
\hline
  \multirow{1}{*}{05} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.17} &
    \texttt{i <= j} &
    2 &
    1 &
    0.16 &
    0.00 \\
\hline
  \multirow{2}{*}{06} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.67} &
    \texttt{x <= y} &
    1 &
    0 &
    0.30 &
    0.00 \\
    & & &
    \texttt{y <= x} &
    1 &
    0 &
    0.29 &
    0.00 \\
\hline
  \multirow{2}{*}{07} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{1.40} &
    \texttt{a + b <= 3*n} &
    3 &
    2 &
    1.34 &
    0.00 \\
    & & &
    \texttt{3*n <= a + b} &
    2 &
    1 &
    0.05 &
    0.00 \\
\hline
  \multirow{1}{*}{08} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{1.06} &
    \texttt{3 <= y} &
    2 &
    1 &
    1.05 &
    0.00 \\
\hline
  \multirow{1}{*}{09} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{18.60} &
    \texttt{0 <= k} &
    16 &
    3 &
    2.61 &
    15.60 \\
\hline
  \multirow{2}{*}{10} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{2.15} &
    \texttt{x <= y} &
    1 &
    0 &
    0.85 &
    0.00 \\
    & & &
    \texttt{y <= x} &
    1 &
    0 &
    0.78 &
    0.00 \\
\hline
  \multirow{2}{*}{11} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{5.47} &
    % \texttt{j <= 200} &
    % 2 &                  First try
    % 1 &
    % 0.00 &
    % 3.23 \\
    % & & &
    \texttt{j <= 200} &
    2 &        % 2 &       Second try
    1 &        % 1 &    
    1.11   &   % 1.11 & 
    4.35 \\    % 1.12 \\
    & & &      % & & &  
    \texttt{200 <= j} &
    2 &
    1 &
    0.02 &
    0.00 \\
\hline
  \multirow{1}{*}{12} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{8.20} &
    \texttt{y <= 4} &
    9 &
    3 &
    3.43 &
    4.58 \\
\hline
  \multirow{2}{*}{13} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{4.05} &
    \texttt{j <= 2 + 2*k} &
    6 &
    2 &
    3.25 &
    0.56 \\
    & & &
    \texttt{2 + 2*k <= j} &
    3 &
    1 &
    0.09 &
    0.00 \\
\hline
  \multirow{2}{*}{14} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{2.38} &
    \texttt{0 <= a + m} &
    2 &
    1 &
    0.03 &
    1.12 \\
    & & &
    \texttt{a <= m} &
    2 &
    1 &
    0.05 &
    1.18 \\
\hline
  \multirow{1}{*}{15} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{1.13} &
    \texttt{0 <= k} &
    2 &
    1 &
    0.02 &
    1.11 \\
\hline
  \multirow{2}{*}{16} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.02} &
    \texttt{y <=0} &
    2 &
    1 &
    0.01 &
    0.00 \\
    & & &
    \texttt{0 <= y} &
    2 &
    1 &
    0.01 &
    0.00 \\
\hline
  \multirow{1}{*}{17} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{1.26} &
    \texttt{n <= k} &
    3 &
    2 &
    0.14 &
    1.10 \\
\hline
  \multirow{2}{*}{18} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{8.37} &
    \texttt{j <= 100} &
    6 &
    2 &
    4.05 &
    3.74 \\
    & & &
    \texttt{100 <= j} &
    3 &
    1 &
    0.44 &
    0.00 \\
\hline
  \multirow{2}{*}{19} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{7.23} &
    \texttt{y <= n} &
    6 &
    2 &
    3.64 &
    2.22 \\
    & & &
    \texttt{n <= y} &
    3 &
    2 &
    1.10 &
    0.00 \\
\hline
  \multirow{4}{*}{20} &
  \multirow{4}{*}{\checkmark} &
  \multirow{4}{*}{5.55} &
    \texttt{x + y <= k} &
    2 &
    1 &
    0.04 &
    0.00 \\
    & & &
    \texttt{k <= x + y} &
    2 &
    1 &
    0.03 &
    0.00 \\
    & & &
    \texttt{0 <= m} &
    4 &
    3 &
    1.19 &
    0.00 \\
    & & &
    \texttt{1 + m <= n} &
    7 &
    3 &
    1.64 &
    2.25 \\
\hline
  \multirow{1}{*}{21} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.03} &
    \texttt{1 + n <= k} &
    2 &
    1 &
    0.03 &
    0.00 \\
\hline
  \multirow{4}{*}{22} &
  \multirow{4}{*}{\checkmark} &
  \multirow{4}{*}{0.16} &
    \texttt{x <= y} &
    1 &
    0 &
    0.01 &
    0.00 \\
    & & &
    \texttt{y <= x} &
    1 &
    0 &
    0.11 &
    0.00 \\
    & & &
    \texttt{y <= z} &
    1 &
    0 &
    0.02 &
    0.00 \\
    & & &
    \texttt{z <= y} &
    1 &
    0 &
    0.01 &
    0.00 \\
\hline
  \multirow{1}{*}{23} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{1.05} &
    \texttt{0 <= sum} &
    3 &
    2 &
    1.03 &
    0.00 \\
\hline
  \multirow{1}{*}{24} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.48} &
    \texttt{i <= k} &
    2 &
    1 &
    0.39 &
    0.07 \\
\hline
  \multirow{1}{*}{25} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.19} &
    \texttt{j <= i} &
    1 &
    0 &
    0.15 &
    0.02 \\
\hline
  \multirow{2}{*}{26} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.88} &
    \texttt{x <= y} &
    1 &
    0 &
    0.40 &
    0.00 \\
    & & &
    \texttt{y <= x} &
    1 &
    0 &
    0.37 &
    0.00 \\
\hline
  \multirow{1}{*}{27} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.04} &
    \texttt{1 <= k} &
    1 &
    0 &
    0.04 &
    0.00 \\
\hline
  \multirow{2}{*}{28} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.05} &
    \texttt{y <= 0} &
    3 &
    2 &
    0.02 &
    0.00 \\
    & & &
    \texttt{0 <= y} &
    3 &
    2 &
    0.02 &
    0.00 \\
\hline
  \multirow{2}{*}{29} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.23} &
    \texttt{a + c <= b + d} &
    1 &
    0 &
    0.03 &
    0.00 \\
    & & &
    \texttt{b + d <= a + c} &
    1 &
    0 &
    0.18 &
    0.00 \\
\hline
  \multirow{1}{*}{30} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{1.14} &
    \texttt{0 <= c} &
    2 &
    1 &
    0.03 &
    1.11 \\
\hline
  \multirow{2}{*}{31} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{4.11} &
    \texttt{0 <= j} &
    2 &
    1 &
    0.95 &
    1.10 \\
    & & &
    \texttt{i <= 4 + j + n} &
    1 &
    0 &
    0.80 &
    1.11 \\
\hline
  \multirow{1}{*}{32} &
  \multirow{1}{*}{\cross} &
  \multirow{1}{*}{11.00} &
    % \texttt{i <= j} &
    % 5 &                 First try
    % 2 &
    % 2.14 &
    % 3.22 \\
    % & & &
    \texttt{i <= j} &
    5 &         % 5 &     Second try 
    2 &         % 2 &    
    4.3 &      % 2.16 & 
    6.45 \\     % 3.23 \\
\hline
  \multirow{2}{*}{33} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.34} &
    \texttt{x <= y} &
    1 &
    0 &
    0.29 &
    0.00 \\
    & & &
    \texttt{y <= x} &
    1 &
    0 &
    0.03 &
    0.00 \\ \hline
  \multirow{2}{*}{34} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.14} &
    \texttt{x <= 2*y} &
    2 &
    1 &
    0.08 &
    0.00 \\
    & & &
    \texttt{2*y <= x} &
    2 &
    1 &
    0.06 &
    0.00 \\
\hline
\end{longtable}    
\begin{longtable}{|l|c|r|r|r|r|r|r|}
 \hline
  Example & Result & Runtime & Property & Calls & Depth & \textbf{R} (SAT) & \textbf{R} (UNSAT)\\\hline
  \endhead
    \hline
  \multirow{2}{*}{35} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.03} &
    \texttt{x <= n} &
    3 &
    2 &
    0.02 &
    0.00 \\
    & & &
    \texttt{n <= x} &
    2 &
    1 &
    0.00 &
    0.00 \\
\hline
  \multirow{3}{*}{36} &
  \multirow{3}{*}{\checkmark} &
  \multirow{3}{*}{14.89} &
    \texttt{z <= w} &
    2 &
    1 &
    0.78 &
    0.00 \\
    & & &
    \texttt{a <= b} &
    4 &
    2 &
    0.92 &
    4.90 \\
    & & &
    \texttt{b <= a} &
    4 &
    2 &
    1.24 &
    5.77 \\
\hline
  \multirow{2}{*}{37} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{2.17} &
    \texttt{0 <= m} &
    3 &
    2 &
    0.06 &
    2.05 \\
    & & &
    \texttt{1 + m <= n} &
    2 &
    1 &
    0.04 &
    0.00 \\
\hline
  \multirow{2}{*}{38} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{0.15} &
    \texttt{x <= 2*y} &
    2 &
    1 &
    0.07 &
    0.00 \\
    & & &
    \texttt{2*y <= x} &
    2 &
    1 &
    0.07 &
    0.00 \\
\hline
  \multirow{2}{*}{39} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{1.20} &
    \texttt{0 <= glob3\_dc} &
    1 &
    0 &
    0.01 &
    0.00 \\
    & & &
    \texttt{glob3\_dc <= MAXPATHLEN} &
    1 &
    0 &
    0.08 &
    1.11 \\
\hline
  \multirow{2}{*}{40} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{17.74} &
    \texttt{a <= b} &
    11 &
    3 &
    1.17 &
    7.29 \\
    & & &
    \texttt{b <= a} &
    9 &
    3 &
    1.58 &
    5.62 \\
\hline
  \multirow{1}{*}{41} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{1.15} &
    \texttt{1 + 2*n <= z} &
    2 &
    1 &
    0.04 &
    1.11 \\
\hline
  \multirow{1}{*}{42} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{23.21} &
    % \texttt{a \% 2 = 1} &
    % 11 &
    % 2 &
    % 1.48 &
    % 19.88 \\
    % & & &
    \texttt{a \% 2 = 1}\quad \footnote{Assertions consisting of an equality with a modulo operator are internally handled as equalities, not as a conjunction of two inequalities.} &
    4 &
    1 &
    1.87 & % 0.39 &
    19.88 \\ % 0.00
\hline
  \multirow{1}{*}{43} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.01} &
    \texttt{t <= y} &
    1 &
    0 &
    0.01 &
    0.00 \\
\hline
  \multirow{2}{*}{44} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{2.47} &
    \texttt{j <= i} &
    5 &
    2 &
    0.10 &
    1.11 \\
    & & &
    \texttt{i <= j} &
    2 &
    1 &
    0.12 &
    1.11 \\
\hline
  \multirow{2}{*}{45} &
  \multirow{2}{*}{\checkmark} &
  \multirow{2}{*}{1.11} &
    \texttt{x <= y} &
    3 &
    2 &
    0.64 &
    0.00 \\
    & & &
    \texttt{y <= x} &
    1 &
    0 &
    0.35 &
    0.00 \\
\hline
  \multirow{1}{*}{46} &
  \multirow{1}{*}{\checkmark} &
  \multirow{1}{*}{0.83} &
    \texttt{x <= 1} &
    1 &
    0 &
    0.45 &
    0.36 \\
\hline
\end{longtable}

%\end{landscape}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

